Topological Autoencoders

We propose a novel approach for preserving topological structures of the input space in latent representations of autoencoders. Using persistent homology, a technique from topological data analysis, we calculate topological signatures of both the input and latent space to derive a topological loss term. Under weak theoretical assumptions, we construct this loss in a differentiable manner, such that the encoding learns to retain multi-scale connectivity information. We show that our approach is theoretically well-founded and that it exhibits favourable latent representations on a synthetic manifold as well as on real-world image data sets, while preserving low reconstruction errors.

==> tables/main_results_raw.tex <==
%\begin{scriptsize}
{\fontsize{7.5}{9}\selectfont 
\setlength{\tabcolsep}{2pt}
\begin{tabular}{llrrrrrrrr}
\toprule
 Data set &   Method & $\dkl_{0.01}  $ &  $\dkl_{0.1} $ &   $\dkl_{1} $ & $\ell$-Cont   & $\ell$-MRRE &  $\ell$-Trust  & $\ell$-RMSE & Data MSE \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SPHERE DATASET 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}*{\data{Spheres}}     &	Isomap            &                 0.18096  &       \second{0.42048}  &      \second{0.00881}  &         \second{0.79027}  &  \second{0.24573}  &       \second{0.67643}  &  10.37188  &                       --  \\
 & PCA                &        0.33231  &       0.65121  &      0.01530  &        0.74740  &  0.29402  &       0.62557  &  11.76482  &       0.96103  \\
 & TSNE              &        \second{0.15228}  &       0.52722  &      0.01271  &        0.77300  &  \first{0.21740}  &       \first{0.67862}  &   \first{8.05018}  &                       -- \\
 & UMAP              &        0.15687  &       0.61326  &      0.01658  &         0.75153  &  0.24968  &       0.63483  &   \second{9.27009}  &                       --  \\
 & AE           &            0.56571  &       0.74588  &      0.01664  &        0.60663  &  0.34918  &       0.58843  &  13.33061  &       0.81545  \\
 & TopoAE &              \first{0.08504}  &       \first{0.32572}  &      \first{0.00694}  &        \first{0.82200}  &  0.27239  &       0.65775  &  13.45753  &       0.86812  \\
\midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % Fashion MNIST
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{5}*{\data{F-MNIST}} & PCA               &              \first{0.35594}  &       \first{0.05205}  &      \first{0.00069}  &        0.96777  &  0.05744  &       0.91681  &   \first{9.05121}  &       0.18439  \\
& TSNE              &              0.40477  &       0.07095  &      0.00198  &        0.96731  &  \first{0.01962}  &       \second{0.97405}  &  41.25460  &                       -- \\
& UMAP              &                0.42362  &       0.06491  &      0.00163  &       \first{0.98126}  &  0.02867  &       0.95874  &  \second{13.68933}  &                       -- \\
& AE           &       0.47798  &       0.06791  &      0.00125  &        0.96849  &  \second{0.02562}  &       \first{0.97418}  &  20.70674  &       0.10197  \\
& TopoAE &            \second{0.39204}  &       \second{0.05353}  &      \second{0.00100}  &        \second{0.97998}  &  0.03156  &       0.95612  &  20.49122  &       0.12071  \\
 \midrule
 %
 % MNIST
 %
 \multirow{5}*{\data{MNIST}} & PCA               &        0.38876  &       0.16301  &   \second{0.00160}  &          0.90084  &  0.16582  &       0.74546  &  \first{13.17437}  &       0.22269  \\
& TSNE            &        \first{0.27695}  &       \second{0.13266}  &      0.00214  &        0.92101  &  \first{0.03953}  &       \first{0.94624}  &  22.89261  &                       -- \\
&  UMAP              &             \second{0.32063}  &       0.14568  &      0.00234  &        \first{0.93992}  &  \second{0.05109}  &       \second{0.93770}  &  \second{14.61535}  &                       -- \\
&  AE           &               0.61993  &       0.15542  &      0.00156  &       0.91293  &  0.05828  &       0.93699  &  18.18105  &       0.13732  \\
& TopoAE  &              0.34069  &       \first{0.11012}  &      \first{0.00114}  &        \second{0.93210}  &  0.05553  &       0.92844  &  19.57784  &       0.13884  \\
 \midrule
 %
 % CIFAR
 %
\multirow{5}*{\data{CIFAR}} & PCA               &            \second{0.59073}  &       \second{0.01961}  &      \first{0.00023}  &       \first{0.93130}  &  0.11921  &       0.82117  &  \first{17.71567}  &       0.14816  \\
& TSNE              &                 0.62733  &       0.03014  &      0.00073  &        0.90300  &  \first{0.10265}  &       \second{0.86325}  &  \second{25.61099}  &                       -- \\
&  UMAP              &               0.61673  &       0.02562  &      0.00050  &        0.92045  &  0.12680  &       0.81668  &  33.57785  &                       -- \\
&  AE           &                0.66834  &       0.03458  &      0.00062  &        0.85072  &  0.13204  &       \first{0.86359}  &  36.26827  &       0.14030  \\
&  TopoAE  &                 \first{0.55642}  &       \first{0.01879}  &      \second{0.00031}  &         \second{0.92691}  &  \second{0.10809}  &       0.84514  &  37.85914  &       0.13975  \\
\bottomrule
\end{tabular}
%\end{scriptsize}
}
%\select     
     
     
     
     
     
     
     


==> tables/supp_results.tex <==
\begin{tiny}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrrrrrrrr}
\toprule
 Data set &   Method & $\dkl_{0.001}$ & $\dkl_{0.01}$ &  $\dkl_{0.1}$ &   $\dkl_{1}$ & $\dkl_{10}$ & $\ell$-Cont & $\ell$-MRRE &  $\ell$-Trust & $\ell$-RMSE & Data MSE \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SPHERE DATASET 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{6}*{\data{Spheres}}     &	Isomap            &         0.53095 $\pm$ 0.01929 &        0.18096 $\pm$ 0.02547 &       \second{0.42048} $\pm$ 0.00559 &      \second{0.00881} $\pm$ 0.00020 &       \second{0.00009} $\pm$ 0.00000 &  \second{0.79027} $\pm$ 0.00244 &  \second{0.24573} $\pm$ 0.00158 &       \second{0.67643} $\pm$ 0.00323 &  10.37188 $\pm$ 0.22856 &                       --  \\
 & PCA               &         \first{0.22445} $\pm$ 0.00691 &        0.33231 $\pm$ 0.00552 &       0.65121 $\pm$ 0.00256 &      0.01530 $\pm$ 0.00010 &       0.00016 $\pm$ 0.00000 &  0.74740 $\pm$ 0.00140 &  0.29402 $\pm$ 0.00108 &       0.62557 $\pm$ 0.00066 &  11.76482 $\pm$ 0.01460 &       0.96103 $\pm$ 0.00029 \\
 & TSNE              &         \second{0.22794} $\pm$ 0.00722 &        \second{0.15228} $\pm$ 0.00805 &       0.52722 $\pm$ 0.03261 &      0.01271 $\pm$ 0.00058 &       0.00013 $\pm$ 0.00001 &  0.77300 $\pm$ 0.00513 &  \first{0.21740} $\pm$ 0.00472 &       \first{0.67862} $\pm$ 0.00474 &   \first{8.05018} $\pm$ 0.11057 &                       -- \\
 & UMAP              &         0.24752 $\pm$ 0.01917 &        0.15687 $\pm$ 0.00599 &       0.61326 $\pm$ 0.00752 &      0.01658 $\pm$ 0.00028 &       0.00018 $\pm$ 0.00000 &  0.75153 $\pm$ 0.00360 &  0.24968 $\pm$ 0.00094 &       0.63483 $\pm$ 0.00185 &   \second{9.27009} $\pm$ 0.03417 &                       --  \\
 & AE           &         0.28432 $\pm$ 0.02165 &        0.56571 $\pm$ 0.02864 &       0.74588 $\pm$ 0.04323 &      0.01664 $\pm$ 0.00115 &       0.00017 $\pm$ 0.00001 &  0.60663 $\pm$ 0.01685 &  0.34918 $\pm$ 0.00903 &       0.58843 $\pm$ 0.00475 &  13.33061 $\pm$ 0.05198 &       0.81545 $\pm$ 0.00106 \\
 & TopoAE &         0.62765 $\pm$ 0.05415 &        \first{0.08504} $\pm$ 0.01270 &       \first{0.32572} $\pm$ 0.02050 &      \first{0.00694} $\pm$ 0.00055 &       \first{0.00007} $\pm$ 0.00001 &  \first{0.82200} $\pm$ 0.01813 &  0.27239 $\pm$ 0.01108 &       0.65775 $\pm$ 0.01428 &  13.45753 $\pm$ 0.04177 &       0.86812 $\pm$ 0.00074 \\
\midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % Fashion MNIST
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{5}*{\data{Fashion-MNIST}} & PCA               &         0.22559 $\pm$ 0.00011 &        \first{0.35594} $\pm$ 0.00011 &       \first{0.05205} $\pm$ 0.00004 &      \first{0.00069} $\pm$ 0.00000 &       \first{0.00001} $\pm$ 0.00000 &  0.96777 $\pm$ 0.00001 &  0.05744 $\pm$ 0.00001 &       0.91681 $\pm$ 0.00003 &   \first{9.05121} $\pm$ 0.00041 &       0.18439 $\pm$ 0.00000 \\
& TSNE              &         \first{0.03516} $\pm$ 0.00226 &        0.40477 $\pm$ 0.01251 &       0.07095 $\pm$ 0.00962 &      0.00198 $\pm$ 0.00026 &       0.00002 $\pm$ 0.00000 &  0.96731 $\pm$ 0.00268 &  \first{0.01962} $\pm$ 0.00073 &       \second{0.97405} $\pm$ 0.00070 &  41.25460 $\pm$ 0.53671 &                       -- \\
& UMAP              &         \second{0.05069} $\pm$ 0.00238 &        0.42362 $\pm$ 0.00609 &       0.06491 $\pm$ 0.00161 &      0.00163 $\pm$ 0.00005 &       0.00002 $\pm$ 0.00000 &  \first{0.98126} $\pm$ 0.00016 &  0.02867 $\pm$ 0.00034 &       0.95874 $\pm$ 0.00060 &  \second{13.68933} $\pm$ 0.02896 &                       -- \\
& AE           &         0.17177 $\pm$ 0.13603 &        0.47798 $\pm$ 0.09567 &       0.06791 $\pm$ 0.00700 &      0.00125 $\pm$ 0.00017 &       0.00001 $\pm$ 0.00000 &  0.96849 $\pm$ 0.00372 &  \second{0.02562} $\pm$ 0.00217 &       \first{0.97418} $\pm$ 0.00119 &  20.70674 $\pm$ 3.56861 &       0.10197 $\pm$ 0.00222 \\
& TopoAE &         0.11039 $\pm$ 0.02948 &        \second{0.39204} $\pm$ 0.03264 &       \second{0.05353} $\pm$ 0.00959 &      \second{0.00100} $\pm$ 0.00015 &       \second{0.00001} $\pm$ 0.00000 &  \second{0.97998} $\pm$ 0.00194 &  0.03156 $\pm$ 0.00253 &       0.95612 $\pm$ 0.00391 &  20.49122 $\pm$ 0.93206 &       0.12071 $\pm$ 0.00238 \\
 \midrule
 %
 % MNIST
 %
 \multirow{5}*{\data{MNIST}} & PCA               &         0.16754 $\pm$ 0.00051 &        0.38876 $\pm$ 0.00146 &       0.16301 $\pm$ 0.00059 &   0.00160 $\pm$ 0.00001 &        0.00002 $\pm$ 0.00000 &  0.90084 $\pm$ 0.00016 &  0.16582 $\pm$ 0.00022 &       0.74546 $\pm$ 0.00048 &  \first{13.17437} $\pm$ 0.00216 &       0.22269 $\pm$ 0.00002 \\
& TSNE              &         \first{0.03767} $\pm$ 0.00140 &        \first{0.27695} $\pm$ 0.05266 &       \second{0.13266} $\pm$ 0.02362 &      0.00214 $\pm$ 0.00041 &       0.00002 $\pm$ 0.00000 &  0.92101 $\pm$ 0.00288 &  \first{0.03953} $\pm$ 0.00129 &       \first{0.94624} $\pm$ 0.00147 &  22.89261 $\pm$ 0.24373 &                       -- \\
&  UMAP              &         \second{0.07214} $\pm$ 0.00091 &        \second{0.32063} $\pm$ 0.00320 &       0.14568 $\pm$ 0.00207 &      0.00234 $\pm$ 0.00004 &       0.00003 $\pm$ 0.00000 &  \first{0.93992} $\pm$ 0.00066 &  \second{0.05109} $\pm$ 0.00022 &       \second{0.93770} $\pm$ 0.00039 &  \second{14.61535} $\pm$ 0.04332 &                       -- \\
&  AE           &         0.44690 $\pm$ 0.08540 &        0.61993 $\pm$ 0.11742 &       \second{0.15542} $\pm$ 0.02203 &      0.00156 $\pm$ 0.00023 &       \second{0.00002} $\pm$ 0.00000 &  0.91293 $\pm$ 0.00564 &  0.05828 $\pm$ 0.00353 &       0.93699 $\pm$ 0.00262 &  18.18105 $\pm$ 0.21459 &       0.13732 $\pm$ 0.00160 \\
& TopoAE  &         0.32427 $\pm$ 0.03312 &        0.34069 $\pm$ 0.03056 &       \first{0.11012} $\pm$ 0.01069 &      \first{0.00114} $\pm$ 0.00010 &       \first{0.00001} $\pm$ 0.00000 &  \second{0.93210} $\pm$ 0.00132 &  0.05553 $\pm$ 0.00044 &       0.92844 $\pm$ 0.00142 &  19.57784 $\pm$ 0.01812 &       0.13884 $\pm$ 0.00066 \\
 \midrule
 %
 % CIFAR
 %
\multirow{5}*{\data{CIFAR}} & PCA               &         0.27320 $\pm$ 0.00014 &        \second{0.59073} $\pm$ 0.00004 &       \second{0.01961} $\pm$ 0.00001 &      \first{0.00023} $\pm$ 0.00000 &       \first{0.00000} $\pm$ 0.00000 &  \first{0.93130} $\pm$ 0.00000 &  0.11921 $\pm$ 0.00005 &       0.82117 $\pm$ 0.00002 &  \first{17.71567} $\pm$ 0.00084 &       0.14816 $\pm$ 0.00000 \\
& TSNE              &         \first{0.04451} $\pm$ 0.00222 &        0.62733 $\pm$ 0.01427 &       0.03014 $\pm$ 0.00333 &      0.00073 $\pm$ 0.00007 &       0.00001 $\pm$ 0.00000 &  0.90300 $\pm$ 0.00611 &  \first{0.10265} $\pm$ 0.00242 &       \second{0.86325} $\pm$ 0.00151 &  \second{25.61099} $\pm$ 0.11551 &                       -- \\
&  UMAP              &        \second{0.06934} $\pm$ 0.00202 &        0.61673 $\pm$ 0.00052 &       0.02562 $\pm$ 0.00019 &      0.00050 $\pm$ 0.00001 &       0.00001 $\pm$ 0.00000 &  0.92045 $\pm$ 0.00013 &  0.12680 $\pm$ 0.00028 &       0.81668 $\pm$ 0.00019 &  33.57785 $\pm$ 0.00796 &                       -- \\
&  AE           &         0.37737 $\pm$ 0.06507 &        0.66834 $\pm$ 0.02992 &       0.03458 $\pm$ 0.00448 &      0.00062 $\pm$ 0.00021 &       0.00001 $\pm$ 0.00000 &  0.85072 $\pm$ 0.00429 &  0.13204 $\pm$ 0.00316 &       \first{0.86359} $\pm$ 0.00442 &  36.26827 $\pm$ 0.56159 &       0.14030 $\pm$ 0.00190 \\
&  TopoAE  &         0.20877 $\pm$ 0.00951 &        \first{0.55642} $\pm$ 0.00412 &       \first{0.01879} $\pm$ 0.00051 &      \second{0.00031} $\pm$ 0.00002 &       \second{0.00000} $\pm$ 0.00000 &  \second{0.92691} $\pm$ 0.00100 &  \second{0.10809} $\pm$ 0.00210 &       0.84514 $\pm$ 0.00359 &  37.85914 $\pm$ 0.03303 &       0.13975 $\pm$ 0.00171 \\
\bottomrule
\end{tabular}
\end{tiny}
     
     
     
     
     
     
     
     
     
     
     
%     %%%%%%%%%%%%%%%%%%%%%%%%%% 
%     %OLD STUFF BELOW!
%     
%     
%          \multirow{6}*{\data{Spheres}}        &               UMAP &                    0.203729 &                   0.553719 &                  0.014364 &        \first{0.243581} &    \first{8.085793} \\
%             &                PCA &                    0.336197 &                   0.648910 &                  0.015219 &        0.293571 &   11.744817 \\
%             &               t-SNE &                    0.240239 &                   \second{0.397789} &                  0.008836 &        0.248930 &  117.254678 \\
%             &             Isomap &                    \second{0.181289} &                   0.411020 &                  \second{0.008636} &        \second{0.246400} &   \second{10.987272} \\
%    &            AE &                    0.595361 &                   0.662686 &                  0.014052 &        0.325690 &   13.881863 \\
%    &  TopoAE (proposed) &                    \first{0.080047} &                   \first{0.301653} &                  \first{0.006419} &        0.275201 &   11.965862 \\
%    \midrule
%    \multirow{5}*{\data{F-MNIST}} &               UMAP &                    0.407057 &                   0.062517 &                  0.001544 &        \second{0.029811} &   \second{14.046468} \\
%    &                PCA &                    \first{0.355832} &                   \second{0.052051} &                  \first{0.000688} &        0.057441 &    \first{9.051018}  \\
%       &  t-SNE &                        0.441658 &                         0.058529 &                        0.001654 &              0.035838 &        52.010151 \\
%       &            AE &                    0.428957 &                           0.065549 &                  0.001250 &        \first{0.024195} &   21.251947 \\
%    &  TopoAE (proposed) &                    \second{0.369017} &                   \first{0.044519} &                  \second{0.000734} &        0.032117 &   22.252948 \\
%
%    \midrule
%    
%    \multirow{5}*{\data{MNIST}} 
%    & UMAP &                   0.321261 &                   0.138753 &                  0.002514 &        \second{0.052364} &  14.493765 \\
%    & PCA &                    0.389723 &                   0.163971 &                  0.001608 &        0.166031 &  \second{13.175753} \\
%    & t-SNE  &                 \second{0.268983} &                         \second{0.095210} &                        0.001546 &              \first{0.037108} &        18.558259 \\
%    &  AE &                    0.595782 &                   0.099498 &                  \second{0.001325} &        0.084537 &  \first{11.518178}             \\
%   %TODO Update TopoAE!
%   & TopoAE (proposed) &                    \first{0.246625} &                   \first{0.084069} &                  \first{0.000826} &        0.115594 &  18.191449  \\
%\bottomrule
%\end{tabular}
%\end{small}
%



==> tables/table_mnist.tex <==
\begin{tabular}{lllrrrrrr}
\toprule
{} &         dataset &              model &  training.reconstruction\_error &  validation\_density\_kl\_global\_001 &  validation\_density\_kl\_global\_01 &  validation\_density\_kl\_global\_1 &  validation\_mean\_mrre &  validation\_rmse \\
\midrule
0 &  Collected\_runs &  TopoAE (proposed) &                       0.189499 &                          0.244562 &                         0.073685 &                        0.000757 &              0.116212 &        18.116278 \\
1 &  Collected\_runs &               UMAP &                            NaN &                               NaN &                              NaN &                             NaN &              0.056094 &        14.487886 \\
2 &  Collected\_runs &            Vanilla &                       0.174983 &                               NaN &                              NaN &                             NaN &              0.087166 &        11.613313 \\
3 &  Collected\_runs &                PCA &                            NaN &                               NaN &                              NaN &                             NaN &              0.173796 &        13.315254 \\
4 &  Collected\_runs &        TSNE\_prelim &                            NaN &                          0.268983 &                         0.095210 &                        0.001546 &              0.037108 &        18.558259 \\
\bottomrule
\end{tabular}


\begin{tabular}{lllrrrrr}
\toprule
{} & dataset & model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &  test\_rmse \\
\midrule
0 &   MNIST &  UMAP &                    0.321261 &                   0.138753 &                  0.002514 &        0.052364 &  14.493765 \\
\bottomrule
\end{tabular}

==> tables/table_results.tex <==
\begin{small}
\begin{tabular}{llrrrrr}
\toprule
 Data set &              Method &  $\dkl_{0.01}$ &  $\dkl_{0.1}$ &   $\dkl_{1}$ &  MRRE &   RMSE \\
\midrule
     \multirow{6}*{\data{Spheres}}        &               UMAP &                    0.203729 &                   0.553719 &                  0.014364 &        \textbf{0.243581} &    \textbf{8.085793} \\
             &                PCA &                    0.336197 &                   0.648910 &                  0.015219 &        0.293571 &   11.744817 \\
             &               t-SNE &                    0.240239 &                   \textit{0.397789} &                  0.008836 &        0.248930 &  117.254678 \\
             &             Isomap &                    \textit{0.181289} &                   0.411020 &                  \textit{0.008636} &        \textit{0.246400} &   \textit{10.987272} \\
    &            AE &                    0.595361 &                   0.662686 &                  0.014052 &        0.325690 &   13.881863 \\
    &  TopoAE (proposed) &                    \textbf{0.080047} &                   \textbf{0.301653} &                  \textbf{0.006419} &        0.275201 &   11.965862 \\
    \midrule
    \multirow{5}*{\data{F-MNIST}} &               UMAP &                    0.407057 &                   0.062517 &                  0.001544 &        \textit{0.029811} &   \textit{14.046468} \\
    &                PCA &                    \textbf{0.355832} &                   \textit{0.052051} &                  \textbf{0.000688} &        0.057441 &    \textbf{9.051018}  \\
       &  t-SNE &                        0.441658 &                         0.058529 &                        0.001654 &              0.035838 &        52.010151 \\
       &            AE &                    0.428957 &                           0.065549 &                  0.001250 &        \textbf{0.024195} &   21.251947 \\
    &  TopoAE (proposed) &                    \textit{0.369017} &                   \textbf{0.044519} &                  \textit{0.000734} &        0.032117 &   22.252948 \\

    \midrule
    
    \multirow{5}*{\data{MNIST}} 
    & UMAP &                   0.321261 &                   0.138753 &                  0.002514 &        \textit{0.052364} &  14.493765 \\
    & PCA &                    0.389723 &                   0.163971 &                  0.001608 &        0.166031 &  \textit{13.175753} \\
    & t-SNE  &                 \textit{0.268983} &                         \textit{0.095210} &                        0.001546 &              \textbf{0.037108} &        18.558259 \\
    &  AE &                    0.595782 &                   0.099498 &                  \textit{0.001325} &        0.084537 &  \textbf{11.518178}             \\
   %TODO Update TopoAE!
   & TopoAE (proposed) &                    \textbf{0.246625} &                   \textbf{0.084069} &                  \textbf{0.000826} &        0.115594 &  18.191449  \\
\bottomrule
\end{tabular}
\end{small}


% \begin{tabular}{lllrrrrrr}
% \toprule
% {} & dataset &              model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &  test\_rmse &  training.reconstruction\_error \\
% \midrule
% 0 &   MNIST &  TopoAE (proposed) &                    0.246625 &                   0.084069 &                  0.000826 &        0.115594 &  18.191449 &                       0.189499 \\
% \bottomrule
% \end{tabular}


==> tables/table_results_with_reconst.tex <==
\begin{tabular}{lllrrrrrr}
\toprule
{} &       dataset &              model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &   test\_rmse &  training.reconstruction\_error \\
\midrule
0  &        SCurve &            Vanilla &                    0.056538 &                   0.019945 &                  0.001265 &        0.038442 &    1.582880 &                       0.051766 \\
1  &        SCurve &  TopoAE (proposed) &                    0.078835 &                   0.028975 &                  0.001398 &        0.044565 &    0.986490 &                       0.087641 \\
2  &        SCurve &                PCA &                    0.032992 &                   0.020228 &                  0.000768 &        0.100973 &    0.709067 &                            NaN \\
3  &        SCurve &               TSNE &                    0.036500 &                   0.032353 &                  0.001997 &        0.038390 &   51.735474 &                            NaN \\
4  &        SCurve &             Isomap &                    0.016870 &                   0.012698 &                  0.001571 &        0.014569 &    2.509537 &                            NaN \\
5  &        SCurve &               UMAP &                    0.025075 &                   0.012997 &                  0.001633 &        0.017706 &   13.148808 &                            NaN \\
6  &  FashionMNIST &            Vanilla &                    0.428957 &                   0.065549 &                  0.001250 &        0.024195 &   21.251947 &                       0.099783 \\
7  &  FashionMNIST &  TopoAE (proposed) &                    0.369017 &                   0.044519 &                  0.000734 &        0.032117 &   22.252948 &                       0.118748 \\



8  &       Spheres &  TopoAE (proposed) &                    0.080047 &                   0.301653 &                  0.006419 &        0.275201 &   11.965862 &                       0.872397 \\


9  &       Spheres &               UMAP &                    0.203729 &                   0.553719 &                  0.014364 &        0.243581 &    8.085793 &                            NaN \\

10 &       Spheres &            Vanilla &                    0.595361 &                   0.662686 &                  0.014052 &        0.325690 &   13.881863 &                       0.864541 \\


11 &       Spheres &                PCA &                    0.336197 &                   0.648910 &                  0.015219 &        0.293571 &   11.744817 &                            NaN \\
12 &       Spheres &               TSNE &                    0.240239 &                   0.397789 &                  0.008836 &        0.248930 &  117.254678 &                            NaN \\
13 &       Spheres &             Isomap &                    0.181289 &                   0.411020 &                  0.008636 &        0.246400 &   10.987272 &                            NaN \\
\bottomrule
\end{tabular}


==> tables/table_varia.tex <==
\begin{tabular}{llrrr}
\toprule
Data set &              Method &  $\dkl_{001}$ &  $\dkl_{01}$ &  $\dkl_{1}$ \\
\midrule
\multirow{6}*{\data{Spheres}} &  TopoAE (proposed) &                    \textbf{0.080047} &                   \textbf{0.301653} &                  \textbf{0.006419} \\
              &               UMAP &                    0.203729 &                   0.553719 &                  0.014364 \\
              &            AE &                    0.595361 &                   0.662686 &                  0.014052 \\
              &                PCA &                    0.336197 &                   0.648910 &                  0.015219 \\
              &               TSNE &                    0.240239 &                   0.397789 &                  0.008836 \\
              &             Isomap &                    0.181289 &                   0.411020 &                  0.008636 \\
\bottomrule
\end{tabular}




% new with fashion:
\begin{tabular}{lllrrrrrr}
\toprule
{} &       dataset &              model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &   test\_rmse &  training.reconstruc
\midrule
0  &        SCurve &            Vanilla &                    0.056538 &                   0.019945 &                  0.001265 &        0.038442 &    1.582880 &                       0.051766 \\
1  &        SCurve &  TopoAE (proposed) &                    0.078835 &                   0.028975 &                  0.001398 &        0.044565 &    0.986490 &                       0.087641 \\
2  &        SCurve &                PCA &                    0.032992 &                   0.020228 &                  0.000768 &        0.100973 &    0.709067 &                            NaN \\
3  &        SCurve &               TSNE &                    0.036500 &                   0.032353 &                  0.001997 &        0.038390 &   51.735474 &                            NaN \\
4  &        SCurve &             Isomap &                    0.016870 &                   0.012698 &                  0.001571 &        0.014569 &    2.509537 &                            NaN \\
5  &        SCurve &               UMAP &                    0.025075 &                   0.012997 &                  0.001633 &        0.017706 &   13.148808 &                            NaN \\
6  &  FashionMNIST &            Vanilla &                    0.428957 &                   0.065549 &                  0.001250 &        0.024195 &   21.251947 &                       0.099783 \\
7  &  FashionMNIST &                PCA &                    0.355832 &                   0.052051 &                  0.000688 &        0.057441 &    9.051018 &                            NaN \\
8  &  FashionMNIST &  TopoAE (proposed) &                    0.369017 &                   0.044519 &                  0.000734 &        0.032117 &   22.252948 &                       0.118748 \\
9  &  FashionMNIST &               UMAP &                    0.407057 &                   0.062517 &                  0.001544 &        0.029811 &   14.046468 &                            NaN \\
10 &       Spheres &  TopoAE (proposed) &                    0.080047 &                   0.301653 &                  0.006419 &        0.275201 &   11.965862 &                       0.872397 \\
11 &       Spheres &               UMAP &                    0.203729 &                   0.553719 &                  0.014364 &        0.243581 &    8.085793 &                            NaN \\
12 &       Spheres &            Vanilla &                    0.595361 &                   0.662686 &                  0.014052 &        0.325690 &   13.881863 &                       0.864541 \\
13 &       Spheres &                PCA &                    0.336197 &                   0.648910 &                  0.015219 &        0.293571 &   11.744817 &                            NaN \\
14 &       Spheres &               TSNE &                    0.240239 &                   0.397789 &                  0.008836 &        0.248930 &  117.254678 &                            NaN \\
15 &       Spheres &             Isomap &                    0.181289 &                   0.411020 &                  0.008636 &        0.246400 &   10.987272 &                            NaN \\
\bottomrule
\end{tabular}



\begin{tabular}{lllrrrrr}
\toprule
{} &         dataset &        model &  validation\_density\_kl\_global\_001 &  validation\_density\_kl\_global\_01 &  validation\_density\_kl\_global\_1 &  validation\_mean\_mrre &  validation\_rm
\midrule
0 &  Collected\_runs &  TSNE\_prelim &                          0.441658 &                         0.058529 &                        0.001654 &              0.035838 &        52.010151 \\
\bottomrule
\end{tabular}



% MNIST:

begin{tabular}{lllrrrrrr}
\toprule
{} & dataset &    model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &  test\_rmse &  training.reconstruction\_error \\
\midrule
0 &   MNIST &  Vanilla &                    0.595782 &                   0.099498 &                  0.001325 &        0.084537 &  11.518178 &                       0.174983 \\
\bottomrule
etend{tabular}


\begin{tabular}{lllrrrrr}
\toprule
{} & dataset & model &  test\_density\_kl\_global\_001 &  test\_density\_kl\_global\_01 &  test\_density\_kl\_global\_1 &  test\_mean\_mrre &  test\_rmse \\
\midrule
0 &   MNIST &   PCA &                    0.389723 &                   0.163971 &                  0.001608 &        0.166031 &  13.175753 \\
\bottomrule
\end{tabular}
